Robust Graph Meta-learning for Weakly-supervised Few-shot Node Classification

Graphs are widely used to model the relational structure of data, and the research of graph machine learning (ML) has a wide spectrum of applications ranging from drug design in molecular graphs to friendship recommendation in social networks. Prevailing approaches for graph ML typically require abundant labeled instances in achieving satisfactory results, which is commonly infeasible in real-world scenarios since labeled data for newly emerged concepts (e.g., new categorizations of nodes) on graphs is limited. Though meta-learning has been applied to different few-shot graph learning problems, most existing efforts predominately assume that all the data from those seen classes is gold-labeled, while those methods may lose their efficacy when the seen data is weakly-labeled with severe label noise. As such, we aim to investigate a novel problem of weakly-supervised graph meta-learning for improving the model robustness in terms of knowledge transfer. To achieve this goal, we propose a new graph meta-learning framework -- Graph Hallucination Networks (Meta-GHN) in this paper. Based on a new robustness-enhanced episodic training, Meta-GHN is meta-learned to hallucinate clean node representations from weakly-labeled data and extracts highly transferable meta-knowledge, which enables the model to quickly adapt to unseen tasks with few labeled instances. Extensive experiments demonstrate the superiority of Meta-GHN over existing graph meta-learning studies on the task of weakly-supervised few-shot node classification.

==> Abstract.tex <==
Graphs are widely used to model the relational structure of data, and the research of graph machine learning (ML) has a wide spectrum of applications ranging from friendship recommendation in social networks to topic classification in citation graphs. 
Prevailing approaches for graph machine learning (ML) typically require abundant labeled instances in achieving satisfactory results, which is commonly infeasible in real-world scenarios since labeled data for newly emerged concepts (e.g., new categorizations of nodes) on graphs is limited. In order to efficiently learn with a small amount of data on graphs, meta-learning has been investigated in graph ML. By transferring the knowledge learned from previous experiences to new tasks, graph meta-learning approaches have demonstrated promising performance on few-shot graph learning problems. However, most existing efforts predominately assume that all the data from those seen classes is gold-labeled, while those methods may lose their efficacy when the seen data is weakly-labeled with severe label noise. As such, we aim to investigate a novel problem of weakly-supervised graph meta-learning for improving the model robustness in terms of knowledge transfer. To achieve this goal, we propose a new graph meta-learning framework -- Graph Hallucination Networks (Meta-GIN). Based on a new robustness-enhanced episodic training paradigm, Meta-GIN is meta-learned to hallucinate clean node representations from weakly-labeled data and extracts highly transferable meta-knowledge, which enables the model to quickly adapt to unseen tasks with few labeled instances. Extensive experiments demonstrate the superiority of Meta-GIN over existing graph meta-learning studies on the task of weakly-supervised few-shot node classification.


% By constructing a pool of semi-supervised node classification tasks to mimic the real test environment, GPN is able to perform \textit{meta-learning} on an attributed network and derive a highly generalizable model for handling the target classification task. 


% for real-world graphs, a large portion of node classes only contains limited labeled instances, and existing GNNs are unequipped to handle those \textit{few-shot} node classes in the long-tail distribution.




% ranging from  social networks to gene regulatory networks, and computer network security. A growing trend recently is to harness the structure of today’s big data, where much of the data can be represented as graphs. 



% As a prevailing paradigm, graph neural networks (GNNs) have been proposed to tackle different learning tasks on graph-structure data and achieved extensive success.


% identify the informativeness of each labeled instance for building a robust and effective model?

% Specifically, the \textit{network encoder} extracts expressive node representations from the input attributed network, and the \textit{node valuator} estimates the importance scores of labeled nodes in the meantime.


% Yet, this problem remains a challenging problem as we need to address the following questions: (i) How to mitigate the ill effect from weakly-labeled node classes on a graph? (ii) How to further extract and transfer valuable meta-knowledge for solving node classification on unseen nodes with few-shot labels.



==> Problem.tex <==








% Following the commonly used notations, in this paper, we use calligraphic fonts, bold lowercase letters, and bold uppercase letters to denote sets (e.g., $\mathcal{V}$), vectors(e.g., $\mathbf{x}$), and matrices (e.g., $\mathbf{X}$), respectively. The $i^{th}$ row of a matrix $\mathbf{X}$ is denoted by $\mathbf{x}_i$, and the transpose of a matrix $\mathbf{X}$ is represented as $\mathbf{X}^{\mathrm{T}}$. For the other special notations, we will illustrate them in the corresponding sections. 



% Formally, consider an attributed graph $\mathbf{G} = (\mathcal{V}, \mathcal{E}, \mathbf{X})$, where $\mathcal V$ denotes the set of nodes $\{v_1, v_2, \dots, v_n\}$ and $\mathcal{E}$ denotes the set of edges $\{e_1, e_2, \dots, e_m\}$.
% Each node is associated with an
% attribute vector $\mathbf{x}_i \in \mathbb{R}^{d}$ and $\mathbf{X} = [\mathbf{x}_1^{\mathrm{T}}; \mathbf{x}_2^{\mathrm{T}}; \dots; \mathbf{x}_n^{\mathrm{T}}] \in \mathbb{R}^{n \times d}$ denotes all the node features. More concretely, we represent the attributed graph as $\mathbf{G}=(\mathbf{A}, \mathbf{X})$, where  $\mathbf{A} = \{0, 1\}^{n \times n}$ is an adjacency matrix representing the network structure. Accordingly, we formulate the studied problem as follows:









%\smallskip


% m and solves a new few-shot learning
% problem (i.e., meta-testing task, Tmt ) by training on many sampled
% similar tasks (i.e., meta-training tasks)




==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g copyright statements.

==> longref_original.tex <==
@inproceedings{vinyals2016matching,
  title={Matching networks for one shot learning},
  author={Vinyals, Oriol and Blundell, Charles and Lillicrap, Timothy and Wierstra, Daan and others},
  booktitle={Advances in neural information processing systems},
  year={2016}
}

@inproceedings{snell2017prototypical,
  title={Prototypical networks for few-shot learning},
  author={Snell, Jake and Swersky, Kevin and Zemel, Richard},
  booktitle={Advances in neural information processing systems},
  pages={4077--4087},
  year={2017}
}

@inproceedings{sung2018learning,
  title={Learning to compare: Relation network for few-shot learning},
  author={Sung, Flood and Yang, Yongxin and Zhang, Li and Xiang, Tao and Torr, Philip HS and Hospedales, Timothy M},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={1199--1208},
  year={2018}
}

@article{finn2017model,
  title={Model-agnostic meta-learning for fast adaptation of deep networks},
  author={Finn, Chelsea and Abbeel, Pieter and Levine, Sergey},
  journal={arXiv preprint arXiv:1703.03400},
  year={2017}
}

@inproceedings{mishra2018simple,
  title={A simple neural attentive meta-learner},
  author={Mishra, Nikhil and Rohaninejad, Mostafa and Chen, Xi and Abbeel, Pieter},
  booktitle={ICLR},
  year={2018}
}

@article{kipf2016semi,
  title={Semi-supervised classification with graph convolutional networks},
  author={Kipf, Thomas N and Welling, Max},
  journal={arXiv preprint arXiv:1609.02907},
  year={2016}
}

@article{velickovic2017graph,
  title={Graph attention networks},
  author={Veli{\v{c}}kovi{\'c}, Petar and Cucurull, Guillem and Casanova, Arantxa and Romero, Adriana and Lio, Pietro and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1710.10903},
  year={2017}
}

@inproceedings{hamilton2017inductive,
  title={Inductive representation learning on large graphs},
  author={Hamilton, Will and Ying, Zhitao and Leskovec, Jure},
  booktitle={Advances in neural information processing systems},
  pages={1024--1034},
  year={2017}
}

@inproceedings{sinha2015overview,
  title={An overview of microsoft academic service (mas) and applications},
  author={Sinha, Arnab and Shen, Zhihong and Song, Yang and Ma, Hao and Eide, Darrin and Hsu, Bo-June and Wang, Kuansan},
  booktitle={Proceedings of the 24th international conference on world wide web},
  pages={243--246},
  year={2015}
}

@inproceedings{mcauley2015inferring,
  title={Inferring networks of substitutable and complementary products},
  author={McAuley, Julian and Pandey, Rahul and Leskovec, Jure},
  booktitle={Proceedings of the 21th ACM SIGKDD international conference on knowledge discovery and data mining},
  pages={785--794},
  year={2015}
}

@inproceedings{grover2016node2vec,
  title={node2vec: Scalable feature learning for networks},
  author={Grover, Aditya and Leskovec, Jure},
  booktitle={Proceedings of the 22nd ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={855--864},
  year={2016}
}

@inproceedings{perozzi2014deepwalk,
  title={Deepwalk: Online learning of social representations},
  author={Perozzi, Bryan and Al-Rfou, Rami and Skiena, Steven},
  booktitle={Proceedings of the 20th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={701--710},
  year={2014}
}

@inproceedings{ravi2017optimization,
  title={Optimization as a model for few-shot learning},
  author={Ravi, Sachin and Larochelle, Hugo},
  booktitle={ICLR},
  year={2017}
}

@inproceedings{ding2019deep,
  title={Deep anomaly detection on attributed networks},
  author={Ding, Kaize and Li, Jundong and Bhanushali, Rohit and Liu, Huan},
  booktitle={Proceedings of the 2019 SIAM International Conference on Data Mining},
  pages={594--602},
  year={2019},
  organization={SIAM}
}

@book{kleinbaum2002logistic,
  title={Logistic regression},
  author={Kleinbaum, David G and Dietz, K and Gail, M and Klein, Mitchel and Klein, Mitchell},
  year={2002},
  publisher={Springer}
}

@article{scarselli2009graph,
  title={The graph neural network model},
  author={Scarselli, Franco and Gori, Marco and Tsoi, Ah Chung and Hagenbuchner, Markus and Monfardini, Gabriele},
  journal={IEEE Transactions on Neural Networks},
  year={2009}
}

@inproceedings{chang2015heterogeneous,
  title={Heterogeneous network embedding via deep architectures},
  author={Chang, Shiyu and Han, Wei and Tang, Jiliang and Qi, Guo-Jun and Aggarwal, Charu C and Huang, Thomas S},
  booktitle={Proceedings of the 21th ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
  pages={119--128},
  year={2015}
}

@inproceedings{cao2016deep,
  title={Deep neural networks for learning graph representations.},
  author={Cao, Shaosheng and Lu, Wei and Xu, Qiongkai},
  booktitle={AAAI},
  volume={16},
  pages={1145--1152},
  year={2016}
}

@article{bruna2013spectral,
  title={Spectral networks and locally connected networks on graphs},
  author={Bruna, Joan and Zaremba, Wojciech and Szlam, Arthur and LeCun, Yann},
  journal={arXiv preprint arXiv:1312.6203},
  year={2013}
}

@inproceedings{defferrard2016convolutional,
  title={Convolutional neural networks on graphs with fast localized spectral filtering},
  author={Defferrard, Micha{\"e}l and Bresson, Xavier and Vandergheynst, Pierre},
  booktitle={Advances in neural information processing systems},
  pages={3844--3852},
  year={2016}
}

@article{henaff2015deep,
  title={Deep convolutional networks on graph-structured data},
  author={Henaff, Mikael and Bruna, Joan and LeCun, Yann},
  journal={arXiv preprint arXiv:1506.05163},
  year={2015}
}

@inproceedings{tang2008arnetminer,
  title={Arnetminer: extraction and mining of academic social networks},
  author={Tang, Jie and Zhang, Jing and Yao, Limin and Li, Juanzi and Zhang, Li and Su, Zhong},
  booktitle={Proceedings of the 14th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={990--998},
  year={2008}
}

@article{ren2018meta,
  title={Meta-learning for semi-supervised few-shot classification},
  author={Ren, Mengye and Triantafillou, Eleni and Ravi, Sachin and Snell, Jake and Swersky, Kevin and Tenenbaum, Joshua B and Larochelle, Hugo and Zemel, Richard S},
  journal={arXiv preprint arXiv:1803.00676},
  year={2018}
}

@inproceedings{qiao2019transductive,
  title={Transductive episodic-wise adaptive metric for few-shot learning},
  author={Qiao, Limeng and Shi, Yemin and Li, Jia and Wang, Yaowei and Huang, Tiejun and Tian, Yonghong},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={3603--3612},
  year={2019}
}

@article{yao2019graph,
  title={Graph Few-shot Learning via Knowledge Transfer},
  author={Yao, Huaxiu and Zhang, Chuxu and Wei, Ying and Jiang, Meng and Wang, Suhang and Huang, Junzhou and Chawla, Nitesh V and Li, Zhenhui},
  journal={arXiv preprint arXiv:1910.03053},
  year={2019}
}

@inproceedings{zhou2019meta,
  title={Meta-GNN: On Few-shot Node Classification in Graph Meta-learning},
  author={Zhou, Fan and Cao, Chengtai and Zhang, Kunpeng and Trajcevski, Goce and Zhong, Ting and Geng, Ji},
  booktitle={Proceedings of the 28th ACM International Conference on Information and Knowledge Management},
  pages={2357--2360},
  year={2019}
}


@article{li2017meta,
  title={Meta-sgd: Learning to learn quickly for few-shot learning},
  author={Li, Zhenguo and Zhou, Fengwei and Chen, Fei and Li, Hang},
  journal={arXiv preprint arXiv:1707.09835},
  year={2017}
}

@article{qi2011exploring,
  title={Exploring context and content links in social media: A latent space method},
  author={Qi, Guo-Jun and Aggarwal, Charu and Tian, Qi and Ji, Heng and Huang, Thomas},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={34},
  number={5},
  pages={850--862},
  year={2011},
  publisher={IEEE}
}

@article{subramanian2005gene,
  title={Gene set enrichment analysis: a knowledge-based approach for interpreting genome-wide expression profiles},
  author={Subramanian, Aravind and Tamayo, Pablo and Mootha, Vamsi K and Mukherjee, Sayan and Ebert, Benjamin L and Gillette, Michael A and Paulovich, Amanda and Pomeroy, Scott L and Golub, Todd R and Lander, Eric S and others},
  journal={Proceedings of the National Academy of Sciences},
  volume={102},
  number={43},
  pages={15545--15550},
  year={2005},
  publisher={National Acad Sciences}
}

@inproceedings{leskovec2012learning,
  title={Learning to discover social circles in ego networks},
  author={Leskovec, Jure and Mcauley, Julian J},
  booktitle={Advances in neural information processing systems},
  pages={539--547},
  year={2012}
}


@article{borgwardt2005protein,
  title={Protein function prediction via graph kernels},
  author={Borgwardt, Karsten M and Ong, Cheng Soon and Sch{\"o}nauer, Stefan and Vishwanathan, SVN and Smola, Alex J and Kriegel, Hans-Peter},
  journal={Bioinformatics},
  volume={21},
  pages={i47--i56},
  year={2005}
}

@article{xu2018powerful,
  title={How powerful are graph neural networks?},
  author={Xu, Keyulu and Hu, Weihua and Leskovec, Jure and Jegelka, Stefanie},
  journal={arXiv preprint arXiv:1810.00826},
  year={2018}
}

@inproceedings{deng2020meta,
  title={Meta-Learning with Dynamic-Memory-Based Prototypical Network for Few-Shot Event Detection},
  author={Deng, Shumin and Zhang, Ningyu and Kang, Jiaojian and Zhang, Yichi and Zhang, Wei and Chen, Huajun},
  booktitle={Proceedings of the 13th International Conference on Web Search and Data Mining},
  pages={151--159},
  year={2020}
}

@techreport{page1999pagerank,
  title={The pagerank citation ranking: Bringing order to the web.},
  author={Page, Lawrence and Brin, Sergey and Motwani, Rajeev and Winograd, Terry},
  year={1999},
  institution={Stanford InfoLab}
}

@inproceedings{park2019estimating,
  title={Estimating node importance in knowledge graphs using graph neural networks},
  author={Park, Namyong and Kan, Andrey and Dong, Xin Luna and Zhao, Tong and Faloutsos, Christos},
  booktitle={Proceedings of the 25th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
  pages={596--606},
  year={2019}
}

@inproceedings{zhang2019variational,
  title={Variational few-shot learning},
  author={Zhang, Jian and Zhao, Chenglong and Ni, Bingbing and Xu, Minghao and Yang, Xiaokang},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={1685--1694},
  year={2019}
}

@article{garcia2009anomaly,
  title={Anomaly-based network intrusion detection: Techniques, systems and challenges},
  author={Garcia-Teodoro, Pedro and Diaz-Verdejo, Jesus and Maci{\'a}-Fern{\'a}ndez, Gabriel and V{\'a}zquez, Enrique},
  journal={computers \& security},
  year={2009}
}


@inproceedings{zhang2012method,
  title={A method for local community detection by finding core nodes},
  author={Zhang, Tiantian and Wu, Bin},
  booktitle={2012 IEEE/ACM International Conference on Advances in Social Networks Analysis and Mining},
  pages={1171--1176},
  year={2012},
  organization={IEEE}
}

@book{northcutt2002network,
  title={Network intrusion detection},
  author={Northcutt, Stephen and Novak, Judy},
  year={2002},
  publisher={Sams Publishing}
}

@inproceedings{koch2015siamese,
  title={Siamese neural networks for one-shot image recognition},
  author={Koch, Gregory and Zemel, Richard and Salakhutdinov, Ruslan},
  booktitle={ICML deep learning workshop},
  volume={2},
  year={2015},
  organization={Lille}
}

@article{zhang2010understanding,
  title={Understanding bag-of-words model: a statistical framework},
  author={Zhang, Yin and Jin, Rong and Zhou, Zhi-Hua},
  journal={International Journal of Machine Learning and Cybernetics},
  volume={1},
  number={1-4},
  pages={43--52},
  year={2010},
  publisher={Springer}
}

@article{garcia2017few,
  title={Few-shot learning with graph neural networks},
  author={Garcia, Victor and Bruna, Joan},
  journal={arXiv preprint arXiv:1711.04043},
  year={2017}
}

@inproceedings{pennington2014glove,
  title={Glove: Global vectors for word representation},
  author={Pennington, Jeffrey and Socher, Richard and Manning, Christopher D},
  booktitle={Proceedings of the 2014 conference on empirical methods in natural language processing (EMNLP)},
  pages={1532--1543},
  year={2014}
}

@article{wu2019simplifying,
  title={Simplifying graph convolutional networks},
  author={Wu, Felix and Zhang, Tianyi and Souza Jr, Amauri Holanda de and Fifty, Christopher and Yu, Tao and Weinberger, Kilian Q},
  journal={arXiv preprint arXiv:1902.07153},
  year={2019}
}
